Seamless Parametrization in Penner Coordinates

We introduce a conceptually simple and efficient algorithm for seamless parametrization, a key element in constructing quad layouts and texture charts on surfaces. More specifically, we consider the construction of parametrizations with prescribed holonomy signatures i.e., a set of angles at singularities, and rotations along homology loops, preserving which is essential for constructing parametrizations following an input field, as well as for user control of the parametrization structure. Our algorithm performs exceptionally well on a large dataset based on Thingi10k [Zhou and Jacobson 2016], (16156 meshes) as well as on a challenging smaller dataset of [Myles et al. 2014], converging, on average, in 9 iterations. Although the algorithm lacks a formal mathematical guarantee, presented empirical evidence and the connections between convex optimization and closely related algorithms, suggest that a similar formulation can be found for this algorithm in the future.

==> 96-acknowledgments.tex <==
\begin{acks}

\end{acks}

==> 960-math.tex <==
\section{Mathematical considerations}\label{sec:math}

The empirical performance of the algorithm shown in Section~\ref{sec:eval} provides strong evidence that the algorithm is likely to be related to a convex optimization problem: it is highly unlikely that Newton method in a vast majority of cases converges in a near-optimal number of iterations, and in all tested cases converges to a solution (with some caveats for extremely poor quality meshes).  At the same time, three closely related problems do correspond to convex problems: (1) metric optimization of convex objectives described in \citet{capouellez2023metric} subject to angle constraints at vertices, but not on dual loops, (2) the conformal mapping based on scale factors described in \citet{campen2021efficient,gillespie2021discrete}, and (3) the similarity mapping based on a scale-factor 1-form $\psi$ described in \citet{Campen:2017:SimilarityMaps}, with details on the convex functional provided in \citet{Campen:2017:OnSimilarityMaps}.

\paragraph{Comparison to metric optimization.} Our algorithm is very close to the projected gradient algorithm of \citet{capouellez2023metric}, but is different in critical respects. 
The most important difference is the \emph{absence of conformal projection}.  The algorithm of \citet{capouellez2023metric} performs a conformal projection at every state to enforce constraints, which requires an inner loop conformal solve, and more importantly limits the supported constraints to the ones conformal maps support (i.e., not full seamless constraints).  

The second major difference is the absence of explicitly optimized energy. 
While this limits the type of parameterizations the method can produce, at the same time, this has a substantial impact on the algorithm's performance.  Note that the method described in \citet{capouellez2023metric} is inherently a first-order method, with linear convergence.  To apply a second-order Newton method in the setting of constrained optimization, would require second derivatives of the constraints.  However, these are known to be discontinuous.  At the same time, our method is a Newton method with quadratic convergence, and only \emph{first} derivatives of constraints are needed. 

\paragraph{Comparison to conformal mapping.} As described in Section~\ref{sec:overview}, conformal methods, e.g., \citet{campen2021efficient,gillespie2021discrete}, operate in a reduced subspace of Penner coordinates spanned by logarithmic scale factors $u \in \bR^{N_v}$. They minimize the convex function
\[
E(u) = \sum_{T \in M'} \left(2f(\lambda_{a}',\lambda_{b}',\lambda_{c}') - \pi(u_i+u_j+u_k)\right) + \Theta_V^T u
\]
where $a, b, c$ and $i, j, k$ are the edges and vertices of triangle $T'$ respectively (see inset), and $\Theta_V$ are the vertex angle constraints.

\begin{wrapfigure}{l}{0.25\columnwidth}
    \centering
    \includegraphics[width=0.275\columnwidth]{figs/conformal-notation.pdf}
    \label{fig:conformal}
\end{wrapfigure}

As in our method, $(M', \lambda') = \del(M, \lambda)$, where $\lambda_{a} = \lambda_a^0 + u_i + u_j$. $f$ is a per-triangle function involving Milnor's Lobachevsky function \citep[Eq.~(8)]{springborn2008conformal} with the important property that
\[
\frac{\partial  f}{\partial \lambda_{a}'} = \alpha_i^{T'},
\]
and the gradient of $E(u)$ is precisely the vertex constraints.


The iteration of our algorithm is very similar to the Newton iteration used to solve for conformal maps in \citet{gillespie2021discrete} and \citet{campen2021efficient}. There are several important differences: most significantly, as we use $N_e$ length variables, rather than $N_v$ vertex scale factors, we can introduce $V + 2g-1$ holonomy constraints, with degrees of freedom to spare.  As the optimization problem in the conformal case is fully constrained, there is no additional objective optimized directly or indirectly. In our case, each iteration optimizes the deviation from the metric at the previous step.  For this reason, as in \citet{capouellez2023metric}, we evaluate the descent direction and the Jacobian of constraints in Penner coordinates, i.e., with respect to the initial mesh connectivity.

\paragraph{Comparison to similarity mapping.} Similarity methods, e.g., \cite{Campen:2017:SimilarityMaps}, use the energy
\[
E(\psi) = \sum_{T \in M}g(\psi_i^T, \psi_j^T, \psi_k^T) - \Theta^T P^{+} \psi
\]
where $\psi_i^T$ is the value of the closed one-form $\psi$ on the edge of triangle $T$ opposite vertex $i$, and $P^+$ is the pseodoinverse of a matrix formed by coefficient vectors for a basis of closed one-forms. Like $f$, $g$ is a triangle function that depends on Milnor's Lobachevsky function with the corresponding property that
\[
\frac{\partial g}{\partial \psi_i^T} = \alpha_i^T.
\]
Similarity map problems were also considered in a similar context in \citet{rivin1994euclidean}. While these methods were developed in a fixed connectivity setting and a fully rigorous analysis using Penner coordinates is still absent in the literature, the theoretical extension is straightforward.

The mathematical approach used successfully to obtain variational principles for seamless constraints do not directly apply in the metric setting since they produce a scaling one-form that generally will be closed but not necessarily exact and thus not integrable on the surface. However, we note that, intuitively, there are more than enough of degrees of freedom ($N_e$) in the metric $\lambda$ to satisfy $(N_v-1) + 2g$ constraints, and the $N_v - 1$ vertex constraints can be satisfied using the conformal degrees of freedom alone.

\paragraph{Invalid signatures} Unlike in the similarity setting, in the metric setting there are holonomy signatures that theoretically cannot be satisfied by any seamless parameterization. The known invalid signatures are:

\begin{itemize}
    \item any signature with exactly two cones of angles $3\pi/2$ and $5\pi/2$, and
    \item a signature with no cones but nontrivial dual loop holonomy angles, i.e., $k_j^{\ell} \neq 0$.
\end{itemize}

By the discrete Guass-Bonnet theorem, these particular invalid cone prescriptions are only possible on genus 1 surfaces. They can also be interpreted in our Penner coordinate setting. For instance, signatures with no cones correspond to flat tori, and the holonomy of any dual loop on a flat torus is necessarily trivial, so the loop holonomy constraints are redundant with the vertex angle constraints. Verifying that our algorithm produces a valid solution whenever one exists, or identifying cases when it does not work is an important future direction.











==> 98-todo.tex <==

Main points to validate: 
\begin{itemize} 
\item The algorithm works on a broad range of holonomy signatures 

\item Figure~\ref{fig:performance} The algorithm is reasonably efficient 

\item Figure~\ref{fig:myles-examples} The quality of the parametrization produced is high 


\item The quality of the parametrization is not far behind direct optimization, but can be improved once we have a feasible solution.

\item Most other methods we need to discuss compare on the MPZ dataset, however they alter it in various ways. 
\end{itemize}

\begin{itemize}
    \item Tetwild results.
    \begin{itemize}
        \item  Figure~\ref{fig:tetwild-input} Input statistics: histograms of sizes, genus, number of cones, holonomy angles on loops. 
        
        \item  Figure~\ref{fig:tetwild-results}  Histogram of distortion,number of iterations, timing per iteration


        \item  Example images:  high genus (say top 10), high geometric complexity.
    \end{itemize}
    
     \item Figure~\ref{fig:myles-input} Figure~\ref{fig:myles-results} Myles results similar to the above. 

     
     \item Figure~\ref{fig:performance} Performance comparison to the projected grad descent w/o holonomy: number of iterations time per iteration

     
     \item \RC{TODO}  Quality comparison with proj grad descent, based on quality convergence to 1e-10. 
     
     \item Figure~\ref{fig:quality} Quality comparison with symmetric Dirichlet, statistics on refinement (why not run SD to convergence to some threshold?), some examples.
     
     \item Figure~\ref{fig:stress-test} Stress-testing: increasing holonomy number on a loop on a simple example 

     \item \RC{TODO} Impossible examples 3-5 torus, 0-cone torus with nontrivial holonomy - show what happens. 
\end{itemize}


==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> makefile <==
all: *.tex
	latexmk -pdf 00-main
	latexmk -pdf 80-supplemental.tex

clean:
	rm 00-main.blg \
		00-main.log \
		00-main.out \
		00-main.pdf
	rm 80-supplemental.aux \
		80-supplemental.log \
		80-supplemental.out \
		80-supplemental.pdf \
	rm comment.cut missfont.log

